A 78- and 96- minute quasi-periodic gamma-ray oscillations in Sagittarius A*

Using publicly available gamma-rays data from the Fermi satellite and the Fermitools package, we constructed 867-day light curves of Sagittarius A* to search for potential periodicities from 2008 to 2024. By applying statistical and computational inference methods, we used periodograms, a window function, unsupervised machine learning (K-Means), the Markov Chain Monte Carlo method, noise colour analysis, and phase-folding techniques. Additionally, the datasets were fitted with a Jacobi elliptical function using a likelihood approach. In total, 1,463,040 minutes were analysed. This analysis revealed a significant period of enhanced activity lasting ~78 minutes, followed by a quiescent phase of about ~18 minutes, resulting in a total quasi-periodic oscillation (QPO) of around 96 minutes.

==> aas-journals.tex <==
% This file should be included on a main document with an \include option. 
% 
% This is what the AAS defines for bibtex entries.  This file was downloaded
% from the ADS Database (Simbad) here:
% http://adsabs.harvard.edu/abs_doc/aas_macros.html
% 
%   In order to use it go to the ads and ask for a bibtex entry of your
% favourite article...
% 
% Sergio Mendoza
% Cavendish Labs
% Cambridge UK
% Tue Mar 14 20:30:18 GMT 2000
% 
\newcommand{\aj}{Astronomical Journal}
\newcommand{\araa}{Ann. Rev. Ast. \& Ast.}
%\renewcommand{\apj}{ApJ}
%\newcommand{\apj}{Astrophysical Journal}
\newcommand{\apjl}{ApJL}
\newcommand{\apjs}{ApJS}
%\newcommand{\ao}{Applied Optics}
\newcommand{\apss}{Astrophysics and Space Science}
\newcommand{\aap}{Astronomy and Astrophysics}
\newcommand{\aapr}{Astronomy and Astrophysics Reviews}
\newcommand{\aaps}{Astronomy and Astrophysics, Supplement}
\newcommand{\azh}{Astronomicheskii Zhurnal}
\newcommand{\baas}{Bulletin of the AAS}
\newcommand{\jrasc}{Journal of the RAS of Canada}
\newcommand{\memras}{Memoirs of the RAS}
%\newcommand{\mnras}{Monthly Notices of the RAS}
\newcommand{\mnras}{MNRAS}
%\newcommand{\pra}{Physical Review A: General Physics}
%\newcommand{\prb}{Physical Review B: Solid State}
%\newcommand{\prc}{Physical Review C}
%\newcommand{\prd}{Physical Review D}
%\newcommand{\pre}{Physical Review E}
%\newcommand{\prl}{Physical Review Letters}
\newcommand{\pasp}{Publications of the ASP}
\newcommand{\pasj}{Publications of the ASJ}
\newcommand{\qjras}{Quarterly Journal of the RAS}
\newcommand{\skytel}{Sky and Telescope}
\newcommand{\solphys}{Solar Physics}
\newcommand{\sovast}{Soviet Astronomy}
\newcommand{\ssr}{Space Science Reviews}
\newcommand{\zap}{Zeitschrift fuer Astrophysik}
%\newcommand{\nat}{Nature}
\newcommand{\iaucirc}{IAU Cirulars}
\newcommand{\aplett}{Astrophysics Letters}
\newcommand{\apspr}{Astrophysics Space Physics Research}
\newcommand{\bain}{Bulletin Astronomical Institute of the Netherlands}
\newcommand{\fcp}{Fundamental Cosmic Physics}
\newcommand{\gca}{Geochimica Cosmochimica Acta}
\newcommand{\grl}{Geophysics Research Letters}
%\newcommand{\jcp}{Journal of Chemical Physics}
\newcommand{\jgr}{Journal of Geophysics Research}
\newcommand{\jqsrt}{Journal of Quantitiative Spectroscopy and Radiative Transfer}
\newcommand{\memsai}{Mem. Societa Astronomica Italiana}
\newcommand{\nphysa}{Nuclear Physics A}
\newcommand{\physrep}{Physics Reports}
\newcommand{\physscr}{Physica Scripta}
\newcommand{\planss}{Planetary Space Science}
\newcommand{\procspie}{Proceedings of the SPIE}


